The algebra of adjacency patterns: Rees matrix semigroups with reversion

We establish a surprisingly close relationship between universal Horn classes of directed graphs and varieties generated by so-called adjacency semigroups which are Rees matrix semigroups over the trivial group with the unary operation of reversion. In particular, the lattice of subvarieties of the variety generated by adjacency semigroups that are regular unary semigroups is essentially the same as the lattice of universal Horn classes of reflexive directed graphs. A number of examples follow, including a limit variety of regular unary semigroups and finite unary semigroups with NP-hard variety membership problems.

==> pstrics/pst-3d.tex <==
%%
%% This is file `pst-3d.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-3d.dtx  (with options: `pst-3d')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-3d.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-3d.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Package `pst-3d.dtx'
%%
%% Timothy Van Zandt <tvz@nwu.edu> (tvz)
%% Herbert Voss <voss@pstricks.de> (hv)
%%
%% September 03, 2005
%%
%% This file is under the LaTeX Project Public License
%% See CTAN archives in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-3d' is a PSTricks package for tilting and other pseudo-3D tricks
%%


\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey \fi % (hv 2005-09-03)
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
\pst@addfams{pst-3d}
\def\fileversion{1.00}
\def\filedate{2005/09/03}
\message{`PST-3d' v\fileversion, \filedate\space (tvz)}
\csname PSTthreeDLoaded\endcsname
\let\PSTthreeDLoaded\endinput
\pst@def{SetMatrixThreeD}<%
  dup sin /e ED cos /f ED
  /p3 ED /p2 ED /p1 ED
  p1 0 eq
  { /a 0 def /b p2 0 le { 1 } { -1 } ifelse def
    p3 p2 abs
  }
  { p2 0 eq
    { /a p1 0 lt { -1 } { 1 } ifelse def /b 0 def
      p3 p1 abs
    }
    { p1 dup mul p2 dup mul add sqrt dup
      p1 exch div /a ED
      p2 exch div neg /b ED
      p3 p1 a div
    }
    ifelse
  }
  ifelse
  atan dup sin /c ED cos /d ED
  /Matrix3D
  [
    b f mul c a mul e mul sub
    a f mul c b mul e mul add
    d e mul
    b e mul neg c a mul f mul sub
    a e mul neg c b mul f mul add
    d f mul
  ] def>
\pst@def{ProjThreeD}<%
  /z ED /y ED /x ED
  Matrix3D aload pop
  z mul exch y mul add exch x mul add
  4 1 roll
  z mul exch y mul add exch x mul add
  exch>
\pst@def{SetMatrixEmbed}<%
  \tx@SetMatrixThreeD
  Matrix3D aload pop
  /z3 ED /z2 ED /z1 ED /x3 ED /x2 ED /x1 ED
  \tx@SetMatrixThreeD
  [
  Matrix3D aload pop
  z3 mul exch z2 mul add exch z1 mul add 4 1 roll
  z3 mul exch z2 mul add exch z1 mul add
  Matrix3D aload pop
  x3 mul exch x2 mul add exch x1 mul add 4 1 roll
  x3 mul exch x2 mul add exch x1 mul add
  3 -1 roll 3 -1 roll 4 -1 roll 8 -3 roll 3 copy
  x3 mul exch x2 mul add exch x1 mul add 4 1 roll
  z3 mul exch z2 mul add exch z1 mul add
  ]
  concat>
\let\pssetzlength\pssetylength
\define@key[psset]{pst-3d}{viewpoint}{%
  \pst@expandafter\psset@@viewpoint#1 {} {} {} \@nil
  \let\psk@viewpoint\pst@tempg}
\def\psset@@viewpoint#1 #2 #3 #4\@nil{%
  \begingroup
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetzlength\pst@dimc{#3}%
    \xdef\pst@tempg{%
      \pst@number\pst@dima \pst@number\pst@dimb \pst@number\pst@dimc}%
  \endgroup}
\psset[pst-3d]{viewpoint=1 -1 1}
\define@key[psset]{pst-3d}{viewangle}{%
  \pst@getangle{#1}\psk@viewangle}
\psset[pst-3d]{viewangle=0}
\define@key[psset]{pst-3d}{normal}{%
  \pst@expandafter\psset@@viewpoint#1 {} {} {} \@nil
  \let\psk@normal\pst@tempg}
\psset[pst-3d]{normal=0 0 1}
\define@key[psset]{pst-3d}{embedangle}{%
  \pst@getangle{#1}\psk@embedangle}
\psset[pst-3d]{embedangle=0}
\define@key[psset]{pst-3d}{Tshadowsize}{%
  \pst@checknum{#1}\psTshadowsize}
\psset[pst-3d]{Tshadowsize=1}
\define@key[psset]{pst-3d}{Tshadowangle}{%
  \pst@getangle{#1}\psk@Tshadowangle}
\psset[pst-3d]{Tshadowangle=60}
\define@key[psset]{pst-3d}{Tshadowcolor}{%
  \pst@getcolor{#1}\psTshadowcolor}
\psset[pst-3d]{Tshadowcolor=lightgray}

\pst@def{TMSave}<%
  tx@Dict /TMatrix known not { /TMatrix { } def /RAngle { 0 } def } if
  /TMatrix [ TMatrix CM ] cvx def>
\pst@def{TMRestore}<%
  CP /TMatrix [ TMatrix setmatrix ] cvx def moveto>
\pst@def{TMChange}<%
  \tx@TMSave
  /cp [ currentpoint ] cvx def % ??? Check this later.
  CM
  CP T \tx@STV
  CM matrix invertmatrix    % Inv(M')
  matrix concatmatrix       % M Inv(M')
  exch exec
  concat cp moveto>
\def\ThreeDput{\def\pst@par{}\pst@object{ThreeDput}}
\def\ThreeDput@i{\@ifnextchar({\ThreeDput@ii}{\ThreeDput@ii(\z@,\z@,\z@)}}
\def\ThreeDput@ii(#1,#2,#3){%
  \pst@killglue\pst@makebox{\ThreeDput@iii(#1,#2,#3)}}
\def\ThreeDput@iii(#1,#2,#3){%
  \begingroup
    \use@par
    \if@star\pst@starbox\fi
    \pst@makesmall\pst@hbox
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetzlength\pst@dimc{#3}%
    \leavevmode
    \hbox{%
      \pst@Verb{%
        { \pst@number\pst@dima
          \pst@number\pst@dimb
          \pst@number\pst@dimc
          \psk@normal
          \psk@embedangle
          \psk@viewpoint
          \psk@viewangle
          \tx@SetMatrixEmbed
        } \tx@TMChange}%
    \box\pst@hbox
    \pst@Verb{\tx@TMRestore}}%
  \endgroup
  \ignorespaces}
\def\pst@sinandcos#1{%
  \begingroup
    \pst@dima=#1\relax
    \pst@dima=.366022\pst@dima     %Now 1pt=1/32rad
    \pst@dimb=\pst@dima   % dimb->32sin(angle) in pts
    \pst@dimc=32\p@       % dimc->32cos(angle) in pts
    \pst@dimtonum\pst@dima\pst@tempa
    \pst@cntb=\tw@
    \pst@cntc=-\@ne
    \pst@cntg=32
    \loop
    \ifnum\pst@dima>\@cclvi % 256
      \pst@dima=\pst@tempa\pst@dima
      \divide\pst@dima\pst@cntg
      \divide\pst@dima\pst@cntb
      \ifodd\pst@cntb
        \advance\pst@dimb \pst@cntc\pst@dima
        \pst@cntc=-\pst@cntc
      \else
        \advance\pst@dimc by \pst@cntc\pst@dima
      \fi
      \advance\pst@cntb\@ne
    \repeat
    \divide\pst@dimb\pst@cntg
    \divide\pst@dimc\pst@cntg
    \global\pst@dimg\pst@dimb
    \global\pst@dimh\pst@dimc
  \endgroup}
\def\pst@getsinandcos#1{%
  \pst@dimg=100000sp
  \pst@dimg=#1\pst@dimg
  \pst@dimh=36000000sp
  \pst@cntg=0
  \loop
  \ifnum\pst@dimg<\z@
    \advance\pst@dimg\pst@dimh
  \repeat
  \loop
  \ifnum\pst@dimg>\pst@dimh
    \advance\pst@dimg-\pst@dimh
  \repeat
  \pst@dimh=9000000sp
  \def\pst@tempg{%
    \ifnum\pst@dimg<\pst@dimh\else
      \advance\pst@dimg-\pst@dimh
      \advance\pst@cntg\@ne
      \ifnum\pst@cntg>\thr@@ \advance\pst@cntg-4 \fi
      \expandafter\pst@tempg
    \fi}%
  \pst@tempg
  \chardef\pst@quadrant\pst@cntg
  \ifdim\pst@dimg=\z@
    \def\pst@sin{0}%
    \def\pst@cos{1}%
  \else
    \pst@sinandcos\pst@dimg
    \pst@dimtonum\pst@dimg\pst@sin
    \pst@dimtonum\pst@dimh\pst@cos
  \fi%
}
\def\pstilt#1{\pst@makebox{\pstilt@{#1}}}
\def\pstilt@#1{%
  \begingroup
    \leavevmode
    \pst@getsinandcos{#1}%
    \hbox{%
      \ifcase\pst@quadrant
        \kern\pst@cos\dp\pst@hbox
        \pst@dima=\pst@cos\ht\pst@hbox
        \ht\pst@hbox=\pst@sin\ht\pst@hbox
        \dp\pst@hbox=\pst@sin\dp\pst@hbox
      \or
        \kern\pst@sin\ht\pst@hbox
        \pst@dima=\pst@sin\dp\pst@hbox
        \ht\pst@hbox=\pst@cos\ht\pst@hbox
        \dp\pst@hbox=\pst@cos\dp\pst@hbox
      \or
        \kern\pst@cos\ht\pst@hbox
        \pst@dima=\pst@sin\dp\pst@hbox
        \pst@dimg=\pst@sin\ht\pst@hbox
        \ht\pst@hbox=\pst@sin\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \or
        \kern\pst@sin\dp\pst@hbox
        \pst@dima=\pst@sin\ht\pst@hbox
        \pst@dimg=\pst@cos\ht\pst@hbox
        \ht\pst@hbox=\pst@cos\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \fi
      \pst@Verb{%
        { [ 1 0
            \pst@cos\space \ifnum\pst@quadrant>\@ne neg \fi
            \pst@sin\space
            \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
            \ifodd\pst@quadrant exch \fi
            0 0
          ] concat
        } \tx@TMChange}%
      \box\pst@hbox
      \pst@Verb{\tx@TMRestore}%
      \kern\pst@dima}%
  \endgroup}
\def\psTilt#1{\pst@makebox{\psTilt@{#1}}}
\def\psTilt@#1{%
  \begingroup
    \leavevmode
    \pst@getsinandcos{#1}%
    \hbox{%
      \ifodd\pst@quadrant
        \pst@@divide{\dp\pst@hbox}{\pst@cos\p@}%
        \ifnum\pst@quadrant=\thr@@\kern\else\pst@dima=\fi\pst@sin\pst@dimg
        \pst@@divide{\ht\pst@hbox}{\pst@cos\p@}%
        \ifnum\pst@quadrant=\@ne\kern\else\pst@dima=\fi\pst@sin\pst@dimg
      \else
        \ifdim\pst@sin\p@=\z@
          \@pstrickserr{\string\psTilt\space angle cannot be 0 or 180}\@ehpa
          \def\pst@sin{.7071}%
          \def\pst@cos{.7071}%
        \fi
        \pst@@divide{\dp\pst@hbox}{\pst@sin\p@}%
        \ifnum\pst@quadrant=\z@\kern\else\pst@dima=\fi\pst@cos\pst@dimg
        \pst@@divide{\ht\pst@hbox}{\pst@sin\p@}%
        \ifnum\pst@quadrant=\tw@\kern\else\pst@dima=\fi\pst@cos\pst@dimg
      \fi
      \ifnum\pst@quadrant>\@ne
        \pst@dimg=\ht\pst@hbox
        \ht\pst@hbox=\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \fi
      \pst@Verb{%
        { [ 1 0
            \pst@cos\space \pst@sin\space
            \ifodd\pst@quadrant exch \fi
            \tx@Div
            \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
            \ifnum\pst@quadrant>\@ne -1 \else 1 \fi
            0 0
          ] concat
        } \tx@TMChange}%
      \box\pst@hbox
      \pst@Verb{\tx@TMRestore}%
      \kern\pst@dima}%
  \endgroup}
\def\psshadow{\pst@object{psshadow}}
\def\psshadow@i{\pst@makebox{\psshadow@ii}}
\def\psshadow@ii{%
  \begingroup
    \use@par
    \leavevmode
    \pst@getsinandcos{\psk@Tshadowangle}%
    \hbox{%
      \lower\dp\pst@hbox\hbox{%
        \pst@Verb{%
          { [ 1 0
              \pst@cos\space \psTshadowsize mul
              \ifnum\pst@quadrant>\@ne neg \fi
              \pst@sin\space \psTshadowsize mul
              \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
              \ifodd\pst@quadrant exch \fi
              0 0
            ] concat
          } \tx@TMChange}}%
      \hbox to\z@{%   patch 2 (hv), to get it run with xcolor _and_ TeX
       \pst@Verb{ gsave \pst@usecolor\psTshadowcolor}%
       \copy\pst@hbox
       \pst@Verb{ grestore}\hss}%
      \pst@Verb{\tx@TMRestore}%
      \box\pst@hbox}%
  \endgroup}
\catcode`\@=\PstAtCode\relax
\endinput
%%
%% End of file `pst-3d.tex'.


==> pstrics/pst-fr3d.tex <==
%%
%% This is file `pst-fr3d.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-fr3d.dtx  (with options: `pst-fr3d')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-fr3d.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-fr3d.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Package `pst-fr3d.dtx'
%%
%% Denis Girou (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%%
%% February 25, 2002
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-fr3d' is a PSTricks package to draw three dimensional grids
%%   with various customizations.
%%
\csname PstFrameBoxThreeDLoaded\endcsname
\let\PstFrameBoxThreeDLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey \fi
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
\pst@addfams{pst-fr3d}
\def\fileversion{1.01}
\def\filedate{2004/11/14}
\message{`Pst-FrameBox3d' v\fileversion, \filedate\space (Denis Girou)}
\newif\ifPstFrameBoxThreeD@On
\define@key[psset]{pst-fr3d}{FrameBoxThreeDOn}[true]{\@nameuse{PstFrameBoxThreeD@On#1}}
\newif\ifPstFrameBoxThreeD@Opposite
\define@key[psset]{pst-fr3d}{FrameBoxThreeDOpposite}[true]{%
\@nameuse{PstFrameBoxThreeD@Opposite#1}}
\define@key[psset]{pst-fr3d}{FrameBoxThreeDColorHSB}{%
\PstFrameBoxThreeD@ColorHSB@i#1\@nil}
\def\PstFrameBoxThreeD@ColorHSB@i#1\@nil{%
\pst@expandafter\pst@getnumiii{#1} {} {} {} {}\@nil
\edef\PstFrameBoxThreeD@Hue{\pst@tempg}%
\edef\PstFrameBoxThreeD@Saturation{\pst@temph}%
\edef\PstFrameBoxThreeD@Brightness{\pst@tempi}}
\define@key[psset]{pst-fr3d}{FrameBoxThreeDBrightnessDistance}{%
\edef\PstFrameBoxThreeD@BrightnessDistance{#1}}
\psset{%
  FrameBoxThreeDOn=true,FrameBoxThreeDOpposite=false,
  FrameBoxThreeDColorHSB=0 0 0.5,FrameBoxThreeDBrightnessDistance=0.15}%
\def\PstFrameBoxThreeD{%
\@ifnextchar[{\PstFrameBoxThreeD@i}{\PstFrameBoxThreeD@i[]}}
\def\PstFrameBoxThreeD@i[#1]#2{{%
\psset{dimen=middle}%
\psset{#1}%
\ifdim\PstFrameBoxThreeD@Brightness\p@<\z@%
  \def\PstFrameBoxThreeD@FillStyle{none}%
  \def\pst@tempa{0.5}%
\else
  \def\PstFrameBoxThreeD@FillStyle{solid}%
  \def\pst@tempa{\PstFrameBoxThreeD@Brightness}%
\fi
\pst@dimh=\pst@tempa\p@
\advance\pst@dimh\PstFrameBoxThreeD@BrightnessDistance\p@
\pst@dimtonum{\pst@dimh}{\pst@tempb}%
\advance\pst@dimh-\PstFrameBoxThreeD@BrightnessDistance\p@
\advance\pst@dimh-\PstFrameBoxThreeD@BrightnessDistance\p@
\pst@dimtonum{\pst@dimh}{\pst@tempc}%
\ifx\definecolor\@undefined
  \newhsbcolor{PstFrameBoxThreeD@ColorC}{%
    \PstFrameBoxThreeD@Hue \PstFrameBoxThreeD@Saturation \pst@tempa}%
  \ifPstFrameBoxThreeD@On
    \newhsbcolor{PstFrameBoxThreeD@ColorA}{%
      \PstFrameBoxThreeD@Hue \PstFrameBoxThreeD@Saturation \pst@tempc}%
    \newhsbcolor{PstFrameBoxThreeD@ColorB}{%
      \PstFrameBoxThreeD@Hue \PstFrameBoxThreeD@Saturation \pst@tempb}%
  \else
    \newhsbcolor{PstFrameBoxThreeD@ColorA}{%
      \PstFrameBoxThreeD@Hue \PstFrameBoxThreeD@Saturation \pst@tempb}%
    \newhsbcolor{PstFrameBoxThreeD@ColorB}{%
      \PstFrameBoxThreeD@Hue \PstFrameBoxThreeD@Saturation \pst@tempc}%
  \fi
\else
  \definecolor{PstFrameBoxThreeD@ColorC}{hsb}{%
    \PstFrameBoxThreeD@Hue,\PstFrameBoxThreeD@Saturation,\pst@tempa}%
  \ifPstFrameBoxThreeD@On
    \definecolor{PstFrameBoxThreeD@ColorA}{hsb}{%
      \PstFrameBoxThreeD@Hue,\PstFrameBoxThreeD@Saturation,\pst@tempc}%
    \definecolor{PstFrameBoxThreeD@ColorB}{hsb}{%
      \PstFrameBoxThreeD@Hue,\PstFrameBoxThreeD@Saturation,\pst@tempb}%
  \else
    \definecolor{PstFrameBoxThreeD@ColorA}{hsb}{%
      \PstFrameBoxThreeD@Hue,\PstFrameBoxThreeD@Saturation,\pst@tempb}%
    \definecolor{PstFrameBoxThreeD@ColorB}{hsb}{%
      \PstFrameBoxThreeD@Hue,\PstFrameBoxThreeD@Saturation,\pst@tempc}%
  \fi
\fi
\psset{linestyle=none}%
\psframebox[fillstyle=\PstFrameBoxThreeD@FillStyle,
            fillcolor=PstFrameBoxThreeD@ColorC,doubleline=true]{#2}%
\setbox\pst@boxg=\hbox{\psframebox{#2}}%
\setbox\pst@hbox=\hbox{\psframebox[doubleline=true]{#2}}%
\pst@dima=\wd\pst@hbox
\advance\pst@dima-\wd\pst@boxg
\divide\pst@dima\tw@
\pst@dimb=\pst@dima
\advance\pst@dima\wd\pst@boxg
\psset{fillstyle=solid}%
\pspolygon[fillcolor=PstFrameBoxThreeD@ColorA]
          (-\wd\pst@hbox,-\dp\pst@hbox)(-\pst@dima,-\dp\pst@boxg)
          (-\pst@dima,\ht\pst@boxg)(-\wd\pst@hbox,\ht\pst@hbox)
\pspolygon[fillcolor=PstFrameBoxThreeD@ColorB]
          (-\wd\pst@hbox,\ht\pst@hbox)(-\pst@dima,\ht\pst@boxg)
          (-\pst@dimb,\ht\pst@boxg)(0,\ht\pst@hbox)
\ifPstFrameBoxThreeD@Opposite
  \def\pst@tempa{PstFrameBoxThreeD@ColorA}%
  \def\pst@tempb{PstFrameBoxThreeD@ColorB}%
\else
  \def\pst@tempa{PstFrameBoxThreeD@ColorB}%
  \def\pst@tempb{PstFrameBoxThreeD@ColorA}%
\fi
\pspolygon[fillcolor=\pst@tempa]
          (0,-\dp\pst@hbox)(-\pst@dimb,-\dp\pst@boxg)
          (-\pst@dimb,\ht\pst@boxg)(0,\ht\pst@hbox)
\pspolygon[fillcolor=\pst@tempb]
          (-\wd\pst@hbox,-\dp\pst@hbox)(-\pst@dima,-\dp\pst@boxg)
          (-\pst@dimb,-\dp\pst@boxg)(0,-\dp\pst@hbox)
\ifPstFrameBoxThreeD@Opposite
\else
  \psset{linestyle=solid,linewidth=0.2pt,arrows=cc-cc}%
  \psline[linecolor=PstFrameBoxThreeD@ColorA]
         (-\pst@dimb,\ht\pst@boxg)(0,\ht\pst@hbox)
  \psline[linecolor=PstFrameBoxThreeD@ColorB]
         (-\wd\pst@hbox,-\dp\pst@hbox)(-\pst@dima,-\dp\pst@boxg)
\fi}}
\catcode`\@=\PstAtCode\relax
\endinput
%%
%% End of file `pst-fr3d.tex'.

